Ensemble Models for Neural Source Code Summarization of Subroutines

A source code summary of a subroutine is a brief description of that subroutine. Summaries underpin a majority of documentation consumed by programmers, such as the method summaries in JavaDocs. Source code summarization is the task of writing these summaries. At present, most state-of-the-art approaches for code summarization are neural network-based solutions akin to seq2seq, graph2seq, and other encoder-decoder architectures. The input to the encoder is source code, while the decoder helps predict the natural language summary. While these models tend to be similar in structure, evidence is emerging that different models make different contributions to prediction quality -- differences in model performance are orthogonal and complementary rather than uniform over the entire dataset. In this paper, we explore the orthogonal nature of different neural code summarization approaches and propose ensemble models to exploit this orthogonality for better overall performance. We demonstrate that a simple ensemble strategy boosts performance by up to 14.8%, and provide an explanation for this boost. The takeaway from this work is that a relatively small change to the inference procedure in most neural code summarization techniques leads to outsized improvements in prediction quality.

==> approach.tex <==
\section{}

==> rqonetable.tex <==
\begin{figure}[!b]
	{\scriptsize
	\setlength\extrarowheight{14pt} % MIGHT NEED TO TURN THIS BACK OFF LATER
	\begin{tabular}{llllllll}
		          & \rotatebox{90}{approach1} & \rotatebox{90}{approach2} & \rotatebox{90}{approach3} & \rotatebox{90}{approach4} & \rotatebox{90}{approach5} & \rotatebox{90}{approach6} & \rotatebox{90}{approach7} \\
		approach1 & 100 &   &   &   &   &   &   \\
		approach2 & 00.00  & 100 &   &   &   &   &   \\
		approach3 &   & 00.00  & 100 &   &   &   &   \\
		approach4 &   &   & 00.00  & 100 &   &   &   \\
		approach5 &   &   &   & 00.00  & 100 &   &   \\
		approach6 &   &   &   &   & 00.00  & 100 &   \\
		approach7 &   &   &   &   &   & 00.00  & 100
	\end{tabular}
	}
	\vspace{0.2cm}
	\caption{Aggregate BLEU scores for simple ensemble of each pair of baselines.}
\end{figure}


==> rqtwo_old.tex <==
\section{RQ$_2$: Advanced Ensemble Method}

This section describes our methodology for answering RQ$_2$, data, and interpretations.

\subsection{Methodology}

We propose an adaptation to the stacking ensemble technique where the output of the stacking ensemble models, along with the original dataset are provided to a model and a meta-learning aggregator is applied. This allows the ensemble to learn not only from the input data, but also from the output of each trained model. We also propose a new neural-network based aggregation technique which we call The Neuraggregator\textsuperscript{TM}. This is a meta-learning technique that uses an additional attention mechanism between the output distributions to help learn which token in the output vocabulary to predict.

% Here is where you describe more about what we mean by orthogonality and other details about how you answer RQ2.  Basically what you want to do in this section is show that there are sets of methods/functions where each model does best.  You can show a model X vs attendgru and model Y vs attendgru, for instance.  Then you can show that X and Y have some set where they beat attendgru.  Then you can show the overlap between those sets.

% You can compute the softmax values of predictions in these groups.  You can show that the softmax tends to be higher among the methods/functions where a model does better.  This is a mathematical explanation as to why our simple average ensemble works.  You can do a stats test on the groups of softmax values to show the differences are significant, if appropriate to do so.

\subsection{Results}
% \begin{figure*}[t]
% \centering
% \scalebox{0.9}{%
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
%     \hline
%     Model Type&Ensemble Method&Aggregation Method&BA&B1&B2&B3&B4\\\hline
%     Model1 &Method1&Aggregate1&99.99&99.99&99.99&99.99&99.99\\
%     Model1 &Method1&Aggregate1&99.99&99.99&99.99&99.99&99.99\\
%   Model1 &Method1&Aggregate1&99.99&99.99&99.99&99.99&99.99\\
%     Model1 &Method1&Aggregate1&99.99&99.99&99.99&99.99&99.99\\
%     Model1 &Method1&Aggregate1&99.99&99.99&99.99&99.99&99.99\\
%     Model1 &Method1&Aggregate1&99.99&99.99&99.99&99.99&99.99\\
%     \hline
% \end{tabular}
% }
% \caption{Advanced ensemble method results}
% \end{figure*}
% Show tables, pie charts, bar charts, whatever, to build your case.  Refer to the pie chart in RQ2 of Sakib's MSR paper for an example.  The process here will overlap with your TSE paper where you compare ast-attendgru-flat and ast-attendgru-gnn, except that in that paper you don't do anything with ensembling.  Just be careful not to put the exact same results in both papers.  Focus on the ensemble-related stuff here (like the softmax explanation) and keep detailed looks at those two models for that other paper.

% Fill 2ish pages

\newpage






